Reliable Actors with Retry Orchestration

Cloud developers have to build applications that are resilient to failures and interruptions. We advocate for a fault-tolerant programming model for the cloud based on actors, retry orchestration, and tail calls. This model builds upon persistent data stores and messages queues readily available on the cloud. Retry orchestration not only guarantees that (1) failed actor invocations will be retried but also that (2) completed invocations are never repeated and (3) it preserves a strict happen-before relationship across failures within call stacks. Tail calls can break complex tasks into simple steps to minimize re-execution during recovery. We review key application patterns and failure scenarios. We formalize a process calculus to precisely capture the mechanisms of fault tolerance in this model. We briefly describe our implementation. Using an application inspired by a typical enterprise scenario, we validate the functional correctness of our implementation and assess the impact of fault preparedness and recovery on performance.

==> apps.tex <==
This Section presents two applications built using KAR to illustrate
some of its capabilities. First, we use a small example of a fault
tolerant solution to the classic Dining Philosophers problem to
discuss how different fault tolerance patterns can be combined in a
single solution. Second, we describe a more realistic enterprise-style
application that combines both actors and services to build a
multi-component and relatively full-featured showcase application.

\subsection{Dining Philosophers}
\label{sec:apps-dp}
\input{apps-dp}

\subsection{Reefer Container Shipment}
\label{sec:apps-reefer}
\input{apps-reefer}



==> arch.tex <==
The message exchanges in the formal semantics closely match the actual
implementation. However the semantics ignores important practical issues such as
how to group actor instances into application components, how to group messages
into queues, and how to produce and consume messages out of order. We first
consider these questions (\ref{sec:arch-grouping}), then describe the
reconciliation algorithm that is triggered upon failure
(\ref{sec:arch-reconciliation}) and the implementation of the optional
cancellation feature (\ref{sec:arch-cancellation}). Finally, we discuss how KAR
is concretely implemented as a polyglot service mesh on top of Kafka and Redis
(\ref{sec:arch-mesh}) consisting of a common runtime and a collection of
language-specific SDKs (\ref{sec:arch-sdks}).

\subsection{Application Components and Queues}
\label{sec:arch-grouping}

As in a traditional microservice-based architecture, application components may
be dedicated to specific tasks. KAR application components have to declare which
actor type(s) they support. Actors are placed onto compatible components at
instantiation time. The placement decisions are coordinated using a persistent
distributed key-value store with a compare-and-swap operation. Our current
implementation uses Redis. To reduce the frequency of lookups in the
distributed store, each component keeps a private in-memory cache of
lookup results that is invalidated on component failures and
managed with a not recently used replacement policy.

KAR also supports stateless services, formally equivalent to single-use actor
instances. Routing decisions for service invocations are independent from one
another and need not be recorded.

While KAR's formal semantics relies on a single message queue, its
implementation allocates a dedicated message queue for each application
component. The number of queues is dynamically adjusted to account for the
addition or removal of components. Request messages are added to the callee's
queue. Responses are added to the caller's queue for actor.call or to the
callee's queue for actor.tell (tells do not have a waiting caller,
so completion may be recorded in any queue). Sending a message is blocking, waiting for the
message queue to acknowledge the message to guarantee durability. A blocking
invocation is suspended after sending the request message until a matching
response message is received by the caller.

Because of reentrancy and retries, messages are not simply processed by an
application component in order. In each component, a consumer thread listens for
incoming messages. It delivers the response messages to suspended callers and
dispatches the request messages to in-memory per-actor-instance queues, except
for reentrant invocations that bypass the in-memory queues.

KAR's formal semantics makes a convenient but unrealistic assumption about
reliable queues, namely that it is possible to discard or alter messages in the
middle of a queue. Typical production systems like Kafka do not support this. As
a result, the KAR runtime does not enqueue and dequeue messages as formalized,
but instead relies on a much restricted API that permits it to (1) append a
message at the end of a queue and (2) expire messages in bulk.

First, for garbage collection purposes, KAR expires messages after a
configurable delay or above a configurable queue size. These parameters can
be adjusted on a per-application basis to ensure messages are not expired before
use. By default, messages expire after ten minutes.

Second, KAR (a) does not dequeue a request message immediately upon completion
and (b) enqueues all tail calls (to self and others) at the end of the callee's
queue. To ensure a tail call to self runs first, KAR does not release the actor
instance lock and recognizes the tail call as owning the lock (bypassing the
in-memory queue like a reentrant call).

Out-of-order and left-over messages (with respect to the formal semantics) also
have consequences for failure recovery that are dealt with at reconciliation
time.

\subsection{Failures and Reconciliation}
\label{sec:arch-reconciliation}

When an application component fails, KAR needs to decide what to do with the
messages in its queue. KAR enters a reconciliation phase. All components
temporarily stop sending and receiving messages. They reach a consensus on the
list of live components and elect a reconciliation leader. This leader catalogs
unexpired messages. Requests with a matching response or tail call are
discarded. The remaining requests to failed components have to be preserved
since they have not run to completion yet. KAR invalidates all placement
decisions for all actor instances placed onto the failed components and
eagerly chooses a replacement component for each failed actor instance with
pending requests. The request messages are then appended to the queues of the
selected  components. Not all actor types however may be supported by live
components. KAR enqueues the matching requests in a queue dedicated to
unavailable actor types. KAR revisits this queue when new components are added
to the application. This queue is logically the same as a failed component
queue.

By construction, reconciliation has to copy every request to failed actor
instances. We take this opportunity to fix the ordering ``mistakes'' we made
earlier. We move tail calls to the correct positions according to the formal
semantics to achieve the proper execution order upon reconciliation.

Request messages for blocking calls (actor.call) include the request id for the
caller. Reconciliation identifies every request with a pending blocking nested
call by transposing the callee-caller map. It alters the copy of the request
message to include the id of the pending callee. When the request is received,
the presence of this optional callee id instructs the consumer thread to postpone the
retry of the request until a response from the callee is received, hence
implementing happen-before constraint of the formal semantics.

%Because callers may migrate from failed application components to live ones, we
%need callees to dynamically decide which component to respond to. Before
%sending a response message, KAR checks that the component for the original
%callee is still alive using the component id embedded in the message and the
%set of live components established at the last reconciliation. If not, the
%runtime queries the distributed placement table. 

At the end of reconciliation, the queues attached to failed components can be
discarded or flushed for later reuse. A failure during reconciliation simply
restarts the reconciliation algorithm. Request messages that have already been
copied into the queues of live application components are skipped.

Reconciliation is relatively expensive as it requires KAR to temporarily suspend
the application and scan recent messages. But reconciliation is only one aspect of
failure detection and recovery. To avoid false positives,
Kafka recommends and defaults to a 10s grace period of missed heartbeats before
reporting a failure. Given this time scale,  there is
room for a relatively involved reconciliation algorithm.
In Section~\ref{sec:apps-reefer} we observe
experimentally that, in our application scenario, reconciliation is responsible
for just under half of the total time of an outage.

%Having considered several possible implementations of KAR semantics on top of
%Kafka, we decided to adopt reconciliation for multiple reasons. First, in
%contrast to, say, relying on Kafka transactions to pull a request and push a
%response message at once, reconciliation does not incur any overhead during
%normal execution (in-between failures). Second, as we further optimize
%reconciliation, in particular by more precisely controlling the scope of the
%scan with checkpoints, we expect this recovery time will significantly shorten.

\subsection{Cancellation}
\label{sec:arch-cancellation}

To implement the optional cancellation feature, KAR checks that the caller's
component is alive before beginning the execution of the callee, using the list
of live application components established as part of the most recent
reconciliation. A callee with a failed caller is not executed.

This implementation does not reflect failures in real time, hence does not
strictly obey the formal semantics. A callee cannot execute once the failure of
the caller has been detected. Since the caller cannot be retried before the
detection of the failure either, and because failure detection is a consensus,
the happen-before relationship still holds.

\subsection{Service Mesh Architecture}
\label{sec:arch-mesh}

Beyond fault-tolerance, KAR has additional traits that
support cloud application development:
\begin{itemize}
\item polyglot: KAR is not tied to a particular programming language or
application framework.
\item interoperable: KAR is meant to be interoperable with legacy code and other
systems.
\item scalable: KAR must scale alongside the application it supports, within and
across servers, clusters, data centers, and clouds.
\end{itemize}

Because KAR applications can combine heterogeneous components
implemented using diverse programming languages and middleware frameworks,
we built KAR as an out-of-process
runtime accessed via a REST API augmented by SDKs for select
programming languages. This architecture facilitates interoperability between
KAR actors and traditional REST services. KAR offers a publish-subscribe API
with a vast library of event connectors leveraging Apache
Camel~\cite{camel-website}.

\begin{figure}[t]
  \centering
  \includegraphics[trim=85 10 70 0,clip,width=3.3in]{figures/reefer-app-mesh}
  \caption{The Reefer Container Shipping application deployment (see
    Section~\ref{sec:apps-reefer}) using the KAR service mesh. Each component is
    made up of a KAR runtime process (blue) and an application process
    (green/purple).} \Description{KAR application components are connected over
    the KAR service mesh.}
  \label{fig:mesh}
\end{figure}
\label{page:mesh}

As illustrated in Figure~\ref{fig:mesh}, a running KAR application consists of a
dynamically varying number of process pairs. Each pair consists of one
application process and one runtime process. The two processes run on the same
logical node (same physical host, virtual machine, or Kubernetes pod). %The
%runtime process starts with and stops with the paired application process.

The application and runtime processes communicate via HTTP or HTTP/2. Among
other optimizations, HTTP/2 makes it possible to multiplex thousands of requests
on a single TCP socket. For the KAR programming model, this means supporting
many blocking parallel invocations without the risk of running out of sockets.

The runtime processes communicate with one another using Kafka and coordinate
actor placement in Redis. The Kafka and Redis instances can be private to one
application or shared across many. Limits to KAR's scalability primarily arise
from Redis and Kafka, both scalable, production-grade services with established
track records. KAR's persistent actor state API is also currently implemented on
top of Redis.

Kafka provides not only the reliable message queues, but also the authentication
and discovery mechanisms, the consensus protocol, as well as the health
monitoring and failure detection. Application components authenticate with Kafka
and form a Kafka consumer group for a Kafka topic that is unique to the
application. This topic is dynamically partitioned into independent
queues attached to each application components as described above. Kafka detects
when a component is removed from the group using heartbeats. Kafka waits for the
list of components to stabilize and broadcast the list to all the components,
triggering reconciliation.

\subsection{Common Runtime and Language SDKs}
\label{sec:arch-sdks}

The KAR runtime process is implemented in about 5,000 lines of Go. It combines
the KAR API server and CLI (command line interface). An additional 300
lines defines a mutating webhook for Kubernetes-based deployments.
The KAR CLI or mutating webhook for Kubernetes, automatically create,
configure, and manage the runtime process associated with each application
process.

Although an application process could directly access every capability of its
paired KAR runtime process using its language-neutral REST API, we provide SDKs
for selected languages. Each SDK exposes the core KAR runtime capabilities using
the conventions and idioms of its targeted developer community.  The SDKs
significantly simplify defining an application component containing actors by
providing an actor runtime layer to translate between the REST API used by the
KAR runtime process to invoke actor operations and programmer friendlier
abstractions such as classes and methods. The SDKs encapsulate the KAR
conventions used to encode actor method invocations as REST requests and to
encode/decode REST responses that represent a normal return of a result, a tail
call, or the rethrowing in the calling process of an exception raised by the
callee method. The SDKs also assemble inter-process stack traces to facilitate
debugging.

Our JavaScript SDK targets Node.js developers and is distributed as a \prg{npm}
package. As is typical in server-side Node.js programs, the various SDK methods
uniformly return promises and are intended to be used in an
\prg{async}/\prg{await} style. Since JSON serialization is an integral part of
Node.js, any JavaScript value can be used as an actor method parameter or
result. The SDK provides a hook for registering JavaScript classes as actor
types. By convention, if the class has an \prg{activate} method, it will be
invoked when an actor instance is instantiated.
All methods of actor classes, including field getters, are
re-interpreted as available methods on the actor type defined by the class. The
JavaScript SDK consists of a total of 725 lines: 325 lines of
JavaScript that implements it and 400 lines of
TypeScript interface that docuements it for consumption in IDEs.

Our Java SDKs target enterprise Java developers. As such, they build on standard
J2EE machinery such as \prg{javax.ws.rs} and \prg{javax.json}. Actor types are
implemented by annotating Java classes to identify actor classes and to indicate
which public instance methods are intended to be externally callable.
Serialization and deserialization is supported by requiring actor method
parameters and results to implement \prg{javax.json.JsonValue}. We have built
two Java SDKs: one based on Quarkus~\cite{quarkus-url} and
Mutiny~\cite{mutiny-url} that supports a modern reactive style of programming
and one based on OpenLiberty~\cite{openliberty-url} that supports a more
traditional imperative style. Together the SDKs total 2,850 lines of Java code;
they are packaged as maven artifacts and published to maven central.

Our Python SDK is
built as a standard Python package. To alleviate some of the typical
restrictions of single-threaded Python we use a combination of
HTTPx~\cite{httpx}, Hypercorn~\cite{hypercorn} and FastAPI~\cite{fastapi} to
deliver similar asynchronous execution guarantees to those of the other SDKs
along with support for end-to-end HTTP 2.0 communication. Actors are represented
as Python classes that inherit from a base ``KarActor'' class that acts as an
interface containing the defining features of a KAR actor: actor name, instance
and session IDs. The SDK consists of approximately 650 lines of code.


==> perf.tex <==
This section empirically quantifies the overheads introduced by
reliable message queues and our runtime architecture.
%
Our experimental testbed is a five node Kubernetes v1.22 cluster
provisioned via the managed Kubernetes service of a major public
cloud provider. Each (virtual) worker node has 4 CPUs, 16 GB of
memory, and runs Ubuntu 18.04. The nodes are connected via a 1Gbps
virtual private network. We deploy KAR v1.3.1 on this cluster in conjunction
with three different Kafka and Redis configurations:
{\em ClusterDev}, {\em ClusterProd}, and {\em Managed}.
The {\em Cluster} configurations run deployments of Kafka and Redis
within the Kubernetes cluster.
With {\em ClusterDev}, Kafka and Redis data is not
backed by persistent storage and there is only one replica of each.
With {\em ClusterProd}, Kafka and Redis data is backed by
attached Persistent Volumes that support 1000 IOPS;
Kafka is configured with 3-way replication.
With {\em Managed}, Kafka and Redis
are instantiated using the fully managed production services
offered by the public cloud provider. These managed instances are
provisioned in the same cloud region as the Kubernetes cluster.

Table~\ref{tab:latency} reports the end-to-end latency in milliseconds
of a minimal request-response communication pattern with a small
payload (20 bytes of user data) on these three different KAR system
configurations. We report the median latency of 10,000 iterations. The
two communicating processes are placed on different worker
nodes. The first two columns are baseline measurements that do not
involve the KAR runtime. The {\em Direct HTTP}
column reports the time required for a non-reliable request/response
communication (a {\tt POST} request over an HTTP connection)
between two Node.js processes. The second column, {\em Kafka Only}
isolates the end-to-end latency for two Go processes that send
messages by connecting directly to Kafka using the same Go-based
client as the KAR runtime. The final two columns report the latency
for KAR actor method invocations using the Node.js KAR SDK. {\em Kar
Actor} is the default configuration; {\em KAR Actor (no cache)}
disables the actor placement cache that short circuits
Redis access on most actor method invocations.

\begin{table}[ht]
\centering
\caption{Median round trip message latency in milliseconds}
\label{tab:latency}
  \begin{tabular}{l|r|r|r|r}
  \toprule
               & Direct & Kafka & KAR Actor & KAR Actor  \\
               & HTTP   & Only  &           & (no cache) \\
  \midrule
  ClusterDev   &  2.60  &  4.35 &    6.62   &    7.12    \\
  \midrule
  ClusterProd  &  2.60  & 10.62 &   13.41   &   14.31    \\
  \midrule
  Managed      &  2.60  & 14.56 &   15.80   &   18.06    \\
  \bottomrule
  \end{tabular}
\end{table}

The first conclusion from these numbers is that, unsurprisingly, there
is a measurable cost to communicating through reliable message queues
{\em vs.}  non-resilient direct HTTP connections. When Kafka is
replicated for fault tolerance, the {\em Kafka Only} request-response
latency is $4X$ to $5.6X$ higher than in {\em Direct HTTP}. These
Kafka latencies are comparable with others reported in the literature,
for example \citet{RSM:ecoop2019} reports an end-to-end message
latency of 9 milliseconds using a replicated cloud-deployed Kafka
configuration.  Second, the extra inter-process communication
introduced by the KAR external runtime design and the bookkeeping
associated with actor method invocation only adds modest overheads to
the base cost of using reliable messaging. In the configurations that
we believe are representative of KAR's intended production use cases,
{\em Managed} and {\em ClusterProd}, {\em KAR Actor} incurs less than
$20\%$ additional latency when compared to {\em Kafka Only}. Finally,
we can see that although caching actor placement only provides
a marginal benefit in {\em ClusterDev} and {\em ClusterProd}, it has
more impact in {\em Managed} where the Redis instance is not
co-located in the same Kubernetes cluster as the application
processes.

